Dynamic Maxflow via Dynamic Interior Point Methods

In this paper we provide an algorithm for maintaining a $(1-\epsilon)$-approximate maximum flow in a dynamic, capacitated graph undergoing edge additions. Over a sequence of $m$-additions to an $n$-node graph where every edge has capacity $O(\mathrm{poly}(m))$ our algorithm runs in time $\widehat{O}(m \sqrt{n} \cdot \epsilon^{-1})$. To obtain this result we design dynamic data structures for the more general problem of detecting when the value of the minimum cost circulation in a dynamic graph undergoing edge additions obtains value at most $F$ (exactly) for a given threshold $F$. Over a sequence $m$-additions to an $n$-node graph where every edge has capacity $O(\mathrm{poly}(m))$ and cost $O(\mathrm{poly}(m))$ we solve this thresholded minimum cost flow problem in $\widehat{O}(m \sqrt{n})$. Both of our algorithms succeed with high probability against an adaptive adversary. We obtain these results by dynamizing the recent interior point method used to obtain an almost linear time algorithm for minimum cost flow (Chen, Kyng, Liu, Peng, Probst Gutenberg, Sachdeva 2022), and introducing a new dynamic data structure for maintaining minimum ratio cycles in an undirected graph that succeeds with high probability against adaptive adversaries.

==> combine.tex <==

\section{Combine (WIP)}

\jan{i dont know if we want this to be a seperate section. feel free to copy paste the proof wherever you need it.}

\begin{lemma}[{\cite[Lemma 3.3]{ChenKLPGS22}}]
	\label{lem:flowsum}
There is a deterministic data structure that maintains a dynamic tree $T\subset G=(V,E)$ under insertion/deletion of edges with gradient $\bg$ and length $\bell$, and supports the following operations:
\begin{itemize}
	\item Insert/delete edges $e$ to $T$, under the condition that $T$ is always a tree, or update the gradient $\bg_e$ or lengths $\bell_e$.
	\item For a path of vector $\Delta = \bp(T[u,v])$ for some $u,v\in V$, return $\langle\bg,\Delta\rangle$ and $\langle\bell,|\Delta|\rangle$.
	\item Maintain a flow $\bf\in\R^E$ under operations $\bf\leftarrow\bf+\eta\Delta$ for $\eta\in\R$ and path vector $\Delta=\bp(T[u,v])$, or query the value $\bf_e$.
\end{itemize}	
\end{lemma}

\begin{proof}[Proof of \Cref{thm:inc}]
	We run the IPM \Cref{alg:incremental:ipm} using the data structures of \Cref{thm:minratio,lem:flowsum}.
	For this we let $\kappa = \exp(-O(\log^{7/8}m\log\log m))$ (the parameter from \Cref{thm:minratio}). 
	
	We start with $\bf^{(t)} = 0$ and initialize \Cref{thm:minratio}, $\tilde\bell = \bell_G(\bf)$, $\tilde\bg = \bg_G(\bf)$.
	This gives us $\Ohat(\sqrt{n})$ trees $F_1,...,F_s$ on which we run the data structure of \Cref{lem:flowsum}.
	
	Assume for now that we always have $\tilde\bg,\tilde\bell$ with $\|\mL(\bf^{(t)})^{-1}(\bg-\bg_G(\bf^{(t)}))\|_\infty \le \kappa\alpha/32$ and $\tilde\bell \approx_2\bell_G(\bf^{(t)})$.
	This is true right after initialization and we will later argue that this will also holds true throughout the algorithm.
	
	\paragraph{Finding $\Delta$}
	By \Cref{alg:incremental:ipm} we must attempt to find a circulation $\Delta\in\R^E$ with $\mB^\top\Delta=0$ and $\tilde\bg^\top/\|\tilde\mL\Delta\|_1 \le - \kappa\alpha/4$.
	We attempt to construct such a circle via the \textsc{Query} operation by \Cref{thm:minratio}.
	\Cref{thm:minratio} returns a cycle $\Delta$ with 
	$$
	\frac{\bg^\top\Delta}{\|\tilde\mL\Delta\|_1} \le \kappa \min_{\mB^\top \bc = 0} \frac{\bg^\top\bc}{\|\tilde\mL\bc\|_1}.
	$$
	We can compute the left-hand side using the data structures \Cref{lem:flowsum} as \Cref{thm:minratio} provides the cycle $\Delta$ implicitly as paths on trees.
	If the value is at most $-\kappa\alpha/4$, then we found the desired circulation.
	If the value is larger, then we know
	$$
	\min_{\mB^\top \bc = 0} \frac{\bg^\top\bc}{\|\tilde\mL\bc\|_1} \ge -\alpha/4
	$$
	so we can pause the IPM and tell the adversary that currently no circulation of cost at most $F$ exists in $G$.
	
	\paragraph{Augmenting $\bf^{(t)}$}
	If we found an appropriate cycle $\Delta$ we update the implicit representation of $\bf^{(t)}$ via \Cref{lem:flowsum}.
	For this we directly add $\eta\Delta_e$ to $\bf^{(t)}_e$ for non-tree edges returned by \Cref{thm:minratio}.
	The edges inside trees have their flow implicitly maintained by \Cref{lem:flowsum}.
	
	\paragraph{Handling edge insertions}
	When an edge $e$ is inserted by the adversary, we set $\bf^{(t)}_e = 0$, $\tilde\bell_e = \bell_G(e)$,
	and insert the edge into \Cref{thm:minratio}.
	
	\paragraph{Maintaining $\tilde\bg,\tilde\bell$}
	%We add some flow $\eta\Delta$ to $\bf^{(t)}$ and update $\tilde\bell$ as follows.
	To maintain $\tilde\bg,\tilde\bell$ we maintain some approximate flow $\tilde\bf$.
	Whenever an edge $e$ is removed from the trees $F_1,...,F_s$, we first query the value of the flow on that edge via \Cref{lem:flowsum} before removing the edge from \Cref{lem:flowsum}.
	We then store that flow value in $\tilde\bf_e$. 
	For the non-tree edges $e$ in cycle $\Delta$ we also directly update $\tilde\bf_e \leftarrow \tilde\bf_e + \eta$ so for non tree edges we always have $\tilde\bf_e = \bf^{(t)}_e$.
	For the tree edges $e$ that are in cycle $\Delta$, we set $\tilde\bell_e \leftarrow \bf^{(t)}_e$ with probability $\min\{1, O(\eta\tilde\bell_e^{-1}\log n)\}$. 
	So w.h.p.~we have $|\tilde\mL(\bf_e - \tilde\bf_e)| < 0.01$ on tree edges.
	This sampling can be done efficiently by observing that $\tilde\bell_e \approx_2\tilde\bell_{e'}$ for all edges $e,e'$ on the same tree.
	So we can sample the entire cycle segment on the same tree at once.
	
	We now maintain $\tilde\bell$ by updating $\tilde\bell_e \leftarrow \bell_G(\tilde\bf)_e$ whenever $\tilde\bf_e$ is updated.
	By \Cref{lemma:lengthstability} we have $\tilde\bell\approx_2\bell_G(\bf^{(t)})$.
	
	We also maintain $r \approx_{1+1/(2^{10}\alpha\kappa)} \bc^\top\tilde\bf - F$ by updating $r$ whenever this approximation is violated.
	
	We update $\tilde\bg_e \leftarrow \bg_G(\tilde\bf)_e$ whenever $\tilde\bf_e$ is updated and update all entries of $\tilde\bg$ whenever $r$ is changed.
	By \Cref{lemma:gradientstability} we have $\|\mL(\bf^{(t)})^{-1}(\bg-\bg_G(\bf^{(t)}))\|_\infty \le \kappa/8$.
	
	\paragraph{Complexity}
	We pay $\Ohat(\sqrt{n})$ whenever an entry of $\tilde\bg$ or $\tilde\bell$ is changed to update the data structures \Cref{thm:minratio} and \Cref{lem:flowsum}.
	By \Cref{lemma:residualstability} we update those values for all edges because of a change in $r$ at most $\Ohat(1)$ times over all iterations of the IPM.
	Additionally, we also perform such an update on an edge $e$ when $\tilde\bf_e$ is changed.
	This happens for just $\Ohat(1)$ non-tree edges per iteration as we only have $\Ohat(1)$ non-tree edges in $\Delta$ by \Cref{thm:spanner}.
	For the tree edges, note that we update an edge with probability $\tilde{O}(\eta\tilde\bell_e^{-1})$ where $\eta = \Ohat(1/|\tilde\bg\Delta|) = \Ohat(\|\tilde\mL\Delta\|_1)$.
	So by summing over all edges in $\Delta$, the expected number of updates in one iteration is bounded by $\Ohat(1)$.
\end{proof}
